Improving Spark Application Throughput Via Memory Aware Task Co-location: A Mixture of Experts Approach

Data analytic applications built upon big data processing frameworks such as Apache Spark are an important class of applications. Many of these applications are not latency-sensitive and thus can run as batch jobs in data centers. By running multiple applications on a computing host, task co-location can significantly improve the server utilization and system throughput. However, effective task co-location is a non-trivial task, as it requires an understanding of the computing resource requirement of the co-running applications, in order to determine what tasks, and how many of them, can be co-located. In this paper, we present a mixture-of-experts approach to model the memory behavior of Spark applications. We achieve this by learning, off-line, a range of specialized memory models on a range of typical applications; we then determine at runtime which of the memory models, or experts, best describes the memory behavior of the target application. We show that by accurately estimating the resource level that is needed, a co-location scheme can effectively determine how many applications can be co-located on the same host to improve the system throughput, by taking into consideration the memory and CPU requirements of co-running application tasks. Our technique is applied to a set of representative data analytic applications built upon the Apache Spark framework. We evaluated our approach for system throughput and average normalized turnaround time on a multi-core cluster. Our approach achieves over 83.9% of the performance delivered using an ideal memory predictor. We obtain, on average, 8.69x improvement on system throughput and a 49% reduction on turnaround time over executing application tasks in isolation, which translates to a 1.28x and 1.68x improvement over a state-of-the-art co-location scheme for system throughput and turnaround time respectively.

==> background.tex <==





==> model.tex <==
\section{Predictive Modeling}
% Memory Optimisation Application
\label{sect_model}

%Our predictive model to determine the memory usage function is a K-nearest
%neighbour (KNN) classifier~\cite{Keller1985}. We have exploited a number of modeling techniques, including decision trees and artificial neural networks. We chose KNN because it gives similar
%performance as other alternative techniques and does not require re-training
%when a new memory usage function is added (see also Section~\ref{sec:other_ml}). The input to the model is a set of features that describe an
%application. Its output is a classification label to the memory usage
%function that describes the optimal memory allocation of the target
%application across any input sizes.

Our predictive model to determine the memory usage function is a K-nearest neighbour (KNN) classifier~\cite{Keller1985}.
We have exploited a number of modeling techniques, including decision trees and artificial neural networks (see Section~\ref{sec:other_ml}).
The input to the model is a set of features that describe an application.
Its output is a label to the memory usage function that describes the optimal memory allocation of the target application across any input sizes.


\subsection{Training the Predictor}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth]{fig/training.pdf}
	%\caption{Benchmark comparative between sequential to parallel split memory}
    \vspace{-1mm}
	\caption{The training process.}
    \vspace{-3mm}
	\label{fig:training}
\end{figure}

\begin{figure}[!t]
	\centering
	\subfloat[Sort]{\includegraphics[width=0.22\textwidth]{fig/sortDifferentInputsvsMath.pdf}
	}
    \subfloat[PageRank]{\includegraphics[width=0.22\textwidth]{fig/pagerankDifferentInputsvsMath.pdf}}
    %\vspace{-2mm}
    \caption{ The optimal memory allocation for \texttt{Sort} and \texttt{PageRank} from HiBench for different program inputs.
     %The optimal memory allocation of an application can be accurately described using a mathematical model.
    }
    %\FIXME{Use bigger font sizes in figures.}
    \label{fig:memory_usage}
    \vspace{-3mm}
\end{figure}

Our predictor is built \emph{offline} using a set of training benchmarks.
The built model can then be used to predict the memory usage function for an \emph{unseen} application.
Figure~\ref{fig:training} depicts the process of collecting training data to build a KNN predictor.
This involves finding a mathematical function to describe the optimal memory allocation for each benchmark and collecting feature values of each training program.

During the training process, we run the Spark executor of a training program in isolation on a computing host.
We then profile each training application with different sized  inputs.
For each program input, we vary the amount of memory allocated to the program by changing the Spark configuration.
On average, we evaluate 64 different memory configurations for each program input, showing how the optimal memory allocation changes as a function of the program input size during the training phase.
Next, we try different mathematical modeling techniques, to find out which model best describes how the memory allocation changes as the input size increases for each training program.
In this training phase, we record the memory usage function
used to describe each training program in a database. Our intuition is that the optimal memory allocations for similar programs will be similar (see Section~\ref{sec:functions}).

\vspace{1.5mm}
\noindent \textbf{Example} As an example, consider Figure~\ref{fig:memory_usage} which shows the
optimal memory allocation found through profiling \texttt{HiBench.Sort} and
\texttt{HiBench.PageRank} with different inputs and memory allocations.
The optimal memory allocation of an application can be accurately described using a mathematical model.
We observe that the optimal memory allocation, $y$, of \texttt{HiBench.Sort} and \texttt{HiBench.PageRank} for a given input size, $x$, can be precisely described using an exponential function , $y= m * (1 - e^{(-b*x)})$, $m=5.768$, $b=4.479$ and
a Napierian logarithmic function, $y= m + ln(x)*b $, $m=16.333$, $b=1.79$ respectively.


For the Spark benchmarks used in this work, their optimal memory allocation can be
described with three functions:
$y= m + ln(x)*b$, $y= m * (1 - e^{(-b*x)})$, and
$y = m * x^b$. Table~\ref{table_bench_math} lists the memory usage function per
application used in this work.
This set of models can be extended for other types of applications as needed.
Note that the coefficients $m$ and $b$ are
application-specific. For a new application, these coefficients will be
determined using a few profiling runs.
It is worth mentioning that for the benchmarks used in this work, there is a strong correlation between input size and memory usage. This relationship may change for other types of applications, but our approach allows new functions to be easily added to model new relationships.



One of the key aspects in building a successful predictor is finding the
right features to characterize the input application task. This is described
in the next section. This is followed by sections describing training data
generation and then using our predictor with a nearest neighbour algorithm.

\subsection{Runtime Features}
\label{sect_run_feat}
%As we pointed out in the previous section, the idea of memory predicting is based on finding out the amount of memory used by a task without performing the task for each input size.
%However, this notion only works if the application knows what kind of equation is used by the task.
%Consequently, another mechanism that classifies tasks, without performing a task to each input size, is required.

%\begin{table}[!t]
%	\renewcommand{\arraystretch}{1.3}
%	\caption{Runtime features}
%	\label{table:features}
%    \small
%	\centering
%	\begin{tabular}{ c  l }
%		\toprule
%		\texttt{in} & The number of interrupts per second\\
%		\texttt{cs} & The number of context switches per second \\
%		\texttt{r} & The number of processes waiting for running \\
%		\texttt{bo} & Blocks sent to a block device (blocks/s) \\
%		\texttt{cm} & Number of cache misses\\
%		\bottomrule
%	\end{tabular}
%\vspace{-2mm}
%\end{table}




\noindent\textbf{Feature Selection}
We have evaluated a large number of possible features that can be collected JVM, the Spark framework, and the operating system.
Given the relatively small number of training applications, we need to find a compact set of features in order to build an effective ML model.
Feature selection is performed via two steps described as follows.
We first removed features that carry little or redundant
information.
We then constructed a correlation coefficient matrix to quantify the correlation among
features to remove similar features. The correlation coefficient
takes a value between -1 and 1, the closer the coefficient is to
+/-1, the stronger the correlation between the features. We
removed a feature that has a correlation coefficient greater
than 0.75 (ignore the sign) to any of the already chosen
features.
After these two processes, we found that the set of features listed in Table~\ref{table:features} leads to good overall performance.


%%ZW: I don't think the explaination is convencing, so I rolled back to the previous version!
%We have removed features that carry little or redundant information.
% % % % % % % % % %
%Among the features tested, the runtime features listed in Table~\ref{table:features} have been chosen.
%We found the more \textit{in} or \textit{cs} the less memory is used by the application due to frequent interrupts or context switches.
%Feature \textit{cs} counts the contexts switches per second in the memory. So, if \textit{cs} is higher means that the application has accessed several times to the memory. Becoming a valuable feature for the memory behavior observation.
%A process has to wait for the requested information (feature \textit{r}) in case the memory has not obtained the information yet. If there is a big number of processes waiting there are several changes in the memory, what produces an increment in the memory usage.
%The information sent to a block device (feature \textit{bo}) is information that uses memory space and cannot be deleted until the device is unblocked.
%The higher \textit{bo} becomes, the bigger the memory usage is.
%Cache miss (feature \textit{cm}) is a feature related with the information switched by a process, where the data requested has not been found in the cache memory.
%In conclusion, all these features are decisive to find a relation between two applications and their memory usage function.

% % % % % % % % % %

Some of these features, such as \texttt{in}, \texttt{cs} and \texttt{r}, describe system load while others describe I/O (\texttt{bo}) and memory behavior
(\texttt{cm}) of a program. To collect \texttt{in}, \texttt{cs}, \texttt{r}
and \texttt{bo}, we use \texttt{vmstat}, a system monitoring tool, to sample system load every
\texttt{1} second for up to \texttt{2} minutes, and average the values. We use
\texttt{perf}, a Linux performance profiling
tool, to collect \texttt{cm} from the hardware performance counter.

Furthermore, supervised learning typically works better if the feature values lies in a certain range (e.g. between 0 and 1). Therefore, after collecting the feature values for all training programs, our approach uses the following  Formula~\ref{eq_normalize} to calculate the normalised value, $\overline{X_i}$, for each feature list in Table~\ref{table:features}. %This formula is used to adjust the feature values measured on different scales to a notionally common scale.


\vspace{-3mm}
\begin{equation}
  \overline{X_i}= \frac{X_i - \mu_i}{\sigma_i}
  \label{eq_normalize}
\end{equation}

where $X_i$ is the value for a given feature, $i$; $\mu_i$ and $\sigma_i$ are the mean and the standard deviation of feature $i$, calculated across all training programs.
During runtime deployment, we also use Equation~\ref{eq_normalize} to normalize feature values extracted from an  \emph{unseen} program.




%For this purpose, we investigated which program features can classify the task depending on their memory behavior graph.
%In order to obtain the correct program features, each task is performed with a small input size while our approach stores different performance parameters of the system, such as, CPU metrics, input/output statistics for devices and partitions or java virtual machine among others.
%We examined these performance parameters that could help our application to build the KNN model, and we decided that our predictor uses the features listed in Table~\ref{table:features}.
%
%%In accordance with this investigation, we chose the following performance parameters that our application will use to classify tasks:
%
%%The objective is to create a cluster that contains tasks with memory limits such us Sort, TeraSort, Wordcount and Scan, and another type of cluster containing tasks without memory limits like PageRank.
%
%% %Our predictor uses features to characterize a program's memory behavior. All the features are listed in Table~\ref{table:features}.
%
%
%These performance parameters features are stored in the database of our application.
%\textit{In}, \textit{cs}, \textit{r} and \textit{bo} are collected using the computer system monitoring tool called \textit{vmstat}, while \textit{cm} is obtained the performance analysing tool in Linux called \textit{Perf}.



%Additionally, we save in the database another value originated from the normalisation of this performance parameter, which has been compared to the same performance parameters of other tasks into the database.
%All the normalized parameters implicated in this normalisation process are going to be updated as well.
%The five normalized values of the performance parameters used in the classification process are compared to another task stored in our application using Euclidean distance.
%When this new task has been compared to all tasks stored in our application, our application checks which comparison has obtained the less Euclidean distance.
%Therefore, our application will store the new task in the same cluster as the task with the smallest Euclidean distance.


\subsection{Collect Training Data}



%\begin{figure*}[ht!]
%  \centering
%  % Requires \usepackage{graphicx}
%  \includegraphics[width=0.9\textwidth]{fig/runtime_deploy.pdf}\\
%  \vspace{-2mm}
%  \caption{Predicting optimal memory allocation at runtime.}\label{fig:runtime_predict}
%  \vspace{-3mm}
%\end{figure*}

\begin{figure*}[t!]
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.75\textwidth]{fig/runtime_deploy.pdf}\\
  \vspace{-2mm}
  \caption{Predicting optimal memory allocation at runtime.}\label{fig:runtime_predict}
  \vspace{-5mm}
\end{figure*}


We use the benchmarks from HiBench, BigDataBench, Spark-Perf and Spark-Bench to build a KNN model.
The process of collecting training data is described in Figure~\ref{fig:training}.
To collect training data, we first extract the feature values of each training program by running a single executor in isolation on an unloaded machine, using inputs with an average size of 200M.
Next, we run each training program with different sized inputs and memory configurations to determine the curve of optimal memory allocation.
We then find a memory usage function to closely fit the curve. For each training program, we store its raw and normalised feature values, a md5 checksum of the program binary, and the memory usage function and
its coefficients in a database. Since training is only performed once, it is a \emph{one-off} cost.
In our case the overall training process takes less than a week on a single machine.


\subsection{Runtime Prediction and Task Scheduling \label{sec:runtimedeploy}}
Once we have collected the training data as described above, we can
use a KNN algorithm to predict the optimal memory allocation for any \emph{unseen}
applications and to use the prediction to co-locate application executor tasks at runtime.
To do so, we first predict the optimal memory allocation for each incoming application task and then use the prediction to check if there is enough memory to co-locate tasks and how many tasks of which types can be co-located.

\subsubsection{Prediction}

Figure~\ref{fig:runtime_predict} illustrates the process of runtime prediction. This follows a number of steps:

\textbf{Check if the incoming application is new} \circled{1} - \circled{2}: For each incoming application, we calculate the md5 checksum of the program binary and use the checksum to determine whether the incoming application is new to our system by looking up the checksum in our database. If the program binary has been previously seen, we simply use the memory usage function stored in the database to predict the optimal memory allocation for the given input(step \circled{6}). Otherwise, we follow steps \circled{3} to \circled{5} to predict and instantiate the memory usage function.
It is possible that the memory behavior of an applications may change significantly across inputs even the binary remains unchanged. How to determine such behavior is left as our future work. Conceivably, we could check compare the application's runtime behavior (e.g. IPC or TLB misses) to the expected values to determine if the program's behavior is new to our system.

\textbf{Feature extraction} \circled{3}: If the application binary is new to our system, we profile it on the system alone for up to two minutes.
%an unloaded machine of the data center for up to two minutes.
We extract the feature values (see Table~\ref{table:features}) of the program during the profile run.

\textbf{Model prediction} \circled{4}: To determine the memory usage function of the incoming application, we calculate the Euclidean distance between the input program feature vector and the feature vector of each training program (stored in our database) to find out the \emph{nearest
neighbour}, i.e. the training program that is closest to the input program in the feature space.
%However,
If the closest distance is greater than a threshold (we use 1.0), then we consider that we do not have a training program that is similar enough to the input program.
%For this reason, the program is performed with different input sizes in order to find the mathematical model to represent its memory behavior.
If this is the case, we will profile the program with different input sizes to construct the memory usage function for the input program update our database with the discovered function for future use.
Note that in our experiments we never needed to construct a new function at runtime, because the models built in the training phase are sufficient in describing the set of Spark benchmarks used in this work.
As a result of model prediction, we use the mathematical
model of the nearest neighbour, or the newly created mathematical model, as the memory usage function for the incoming program.
%We also record the optimal memory partition ratio between the
%Spark driver and executors, given by the nearest neighbour.

\textbf{Coefficient instantiation} \circled{5}: After we have determined the
memory usage function for the incoming application, we need to instantiate
the function coefficients (i.e. $m$ and $b$ in this work). For the models used in this
work, this is achieved through performing sample profiling on an unloaded
machine using two different inputs.
%In practice, profiling can be done by using free slots in a data center.
These inputs are supplied by the user or generated through an input generator (which needs to be provided by the user).
%For each input,
%we then vary the Spark memory configuration to find the optimal memory
%allocation.
For an input, $x$, we profile the application using 9 configurations to obtain the optimal memory allocation, $y$.
The 9 configurations generated with memory allocations from 1GB to 32GB, with an incremental step of 4GB (i.e. 1, 4, 8,.., 32 GBs).


Next, we use two sets of $(x, y)$,
collected using two different inputs, to solve the
equations to calculate the values of the model coefficients, $m$ and $b$.
Once we have instantiated the memory usage function, we can use it to predict
the optimal memory allocation for any input size for the
application. Furthermore, we also store the memory usage function for future
use, so that coefficient instantiation only needs to be performed
once.

\textbf{Memory prediction} \circled{6}: Finally, we use the
instantiated function to predict the optimal memory allocation.
Because input data must be submitted together with a Spark task, our framework can acquire the input size from the cluster manager.
%We also use the optimal partition ratio of the closest
%training program to partition memory between the driver and executors
%when they run on the same host.

\subsubsection{Runtime Task Scheduling}
Our application task scheduler built upon YARN~\cite{Vavilapalli:2013:AHY:2523616.2523633}, a task scheduler and resource manager for Spark.
For each newly arriving application
task, we predict its optimal memory allocation for an executor process for a given input as described above. The
application task is then inserted into a task queue according to certain
criteria, e.g. first come first serve (\texttt{FCFS}) or based on task priorities.
Task scheduling will be triggered upon the arrival or completion of a executor task. To do
so, our task scheduler keeps removing a task from the front of the queue, if the available memory of the system can accommodate the optimal memory allocation for the task. If the optimal memory allocation is greater than the physical memory or there is no room to run more than one task, we can simply run the task in isolation using all memory and processor resources.
\emph{Our approach can be used with any task scheduling algorithm}, but in this work we use a \texttt{FCFS} algorithm to evaluate our approach. Furthermore, to minimize the potential thread contention, our scheduler dynamically adjusts the number of threads used by each co-located executor to evenly distribute processor cores across currently-running tasks.


%ZW: I don't think this makes sense. So I comment it out!
%\subsubsection{Runtime overhead}
%%The runtime overhead for an application to be performed for the runtime prediction (steps 1-6) is around
%%In this subsection we will show the runtime overhead per each step.
%
%For 1, 2 and~6 steps, the runtime overhead is so insignificant that it will not affect the runtime overhead of the system.
%In step~3, the runtime overhead is around~2 minutes and 10~seconds to extract the necessary features values of the new application.
%Regarding step~4, the calculation of the Euclidean distance is about 5~seconds.
%In the coefficient instantiation step~(5), the system needs around 35~seconds to perform it.
%On average, the runtime overhead for a new application is approximately 2~minutes and 50~seconds.
%
%If a Spark application is already inserted in the database when it is performed, then our approach executes steps 1, 2 and 6.
%As consequence, the runtime overhead obtained is almost~0.



\input{example} 
